Improving Reliability of Spiking Neural Networks through Fault Aware Threshold Voltage Optimization

Spiking neural networks have made breakthroughs in computer vision by lending themselves to neuromorphic hardware. However, the neuromorphic hardware lacks parallelism and hence, limits the throughput and hardware acceleration of SNNs on edge devices. To address this problem, many systolic-array SNN accelerators (systolicSNNs) have been proposed recently, but their reliability is still a major concern. In this paper, we first extensively analyze the impact of permanent faults on the SystolicSNNs. Then, we present a novel fault mitigation method, i.e., fault-aware threshold voltage optimization in retraining (FalVolt). FalVolt optimizes the threshold voltage for each layer in retraining to achieve the classification accuracy close to the baseline in the presence of faults. To demonstrate the effectiveness of our proposed mitigation, we classify both static (i.e., MNIST) and neuromorphic datasets (i.e., N-MNIST and DVS Gesture) on a 256x256 systolicSNN with stuck-at faults. We empirically show that the classification accuracy of a systolicSNN drops significantly even at extremely low fault rates (as low as 0.012\%). Our proposed FalVolt mitigation method improves the performance of systolicSNNs by enabling them to operate at fault rates of up to 60\%, with a negligible drop in classification accuracy (as low as 0.1\%). Our results show that FalVolt is 2x faster compared to other state-of-the-art techniques common in artificial neural networks (ANNs), such as fault-aware pruning and retraining without threshold voltage optimization.

==> Sections/Sec2_Preliminaries_bak.tex <==
\section{Background}

This section provides a brief overview of the state-of-the-art SNNs and systolicSNNs for better understanding.\\

\indent \textbf{Spiking Neural Networks:} SNNs are referred as bio-inspired neural networks. Their working principle is given as: when a presynaptic neuron emits the action potential i.e., membrane potential $V_{t}$ exceeds a specific $V_{th}$ at time $t$, a post-synaptic spike is generated and then, $V_{t}$ returns to a reset value $V_{rest}$ $<$ $V_{th}$. The postsynaptic spikes travel to postsynaptic neurons and increase or decrease their membrane potentials. Such spiking behavior is usually modeled in terms of synaptic conductance using a well-known leaky integrate-and-fire (LIF) model~\cite{gerstner2014neuronal}. The LIF-based SNNs learn the pre-synaptic weights but employ the fixed membrane time constants. This eventually leads to training with large time steps. Recently, Fang et al. proposed a parametric leaky integrate-and-fire (PLIF) based SNN that learns both pre-synaptic weights and membrane time constants~\cite{fang2021incorporating}. This reduces the time steps especially, in large networks. The PLIF layers are added next to the convolutional layers. In this paper, we use the recent PLIF-based SNN~\cite{fang2021incorporating} for fault vulnerability and mitigation analysis.

\begin{comment}
\begin{figure}[!t]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=0.8\linewidth]{Figs/lif.pdf}
	\vspace{-0.05in}
	\caption{Pre-synaptic and post-synaptic spikes in a spiking neural network (SNN)}
	\label{fig:lif}
	\vspace{-0.2in}
\end{figure}
\end{comment}

\indent \textbf{Systolic-Array SNN Accelerators:} SystolicSNNs exploit the spatial and temporal parallelisms for which spike input and weight data propagate vertically and horizontally across the systolic array, respectively, in time batches. As shown in Fig.~\ref{fig:systolic_array}, the spiking input is first divided into time batches equivalent to time steps and then, each batch is mapped on one column of the systolic array. The input batches and weights pass through the array in a clocked synchronized manner. The systolic array contains a dense $N$x$N$ grid of interconnected PEs. All PEs poses the same design having an adder and selector~\cite{guo2019systolic}~\cite{wang2020sies}. The PE accumulates the weights under the binary spikes logical 1 or 0 and uses an enable signal for the accumulator. Here, the adder needed for accumulation operation is cheaper than the multiplier needed for the multiplier-and-accumulator unit in systolic-array ANN accelerators.

\label{sec:prelim}
\begin{figure}[!h]
	\centering
	\vspace{-0.01in}
	\includegraphics[width=1\linewidth]{Figs/systolic_array.pdf}
	\caption{Systolic-array SNN accelerator (systolicSNN)}
	\label{fig:systolic_array}
	\vspace{-0.195in}
\end{figure}

%==================================================================


==> Sections/Sec3_RelatedWorks.tex <==
\section{Related Works} 
\label{sec:relatedworks}

Recently, Schuman et al. explored the resilience properties of different feed-forward SNNs under dead synapse faults~\cite{schuman2020resilience}. Results show that the classification accuracy drops rapidly with an increase in the fault rates. In another work, Vatajelu et al. presented behavior-level fault injection in a SNN architecture with memristor-based synapse implementation~\cite{vatajelu2019special}. The fault model includes worst case faulty behaviours, such as dead neuron and synapse faults. Results show that a high fault density is required for noticeable decrease in error rate. \textcolor{blue}{These works provide broader implications of large-scale failures in SNNs implemented on neuromorphic hardware.} The hardware faults that hinder the performance of SNNs include permanent faults, such as process variations and stuck-at 0 and 1. El-Sayed et al. analyzed the effect of these faults in a transistor-level design of leaky-integrate-and-fire (LIF) neuron~\cite{el2020spiking}. However, large-scale fault injection experiments require a fault model with higher abstraction to make the simulation traceable. Guo et al. used synaptic stuck-at fault model for analyzing the fault resilience of SNNs trained with different coding schemes~\cite{guo2021neural}. Other state-of-the-art works are focused on bit flips in weight memories~\cite{spyrou2022reliability, putra2021respawn, vidya2022softsnn, venceslai2020neuroattack}. Nevertheless, the impact of stuck-at faults on systolicSNNs has not been studied so far. Recently, Spyrou et al. presented a passive fault tolerance strategy based on the dropout to recover the SNNs from the neuron faults~\cite{spyrou2021neuron}. Mehul et al. proposed an astrocyte self-repair mechanism for stuck-at 0 weights in SNNs~\cite{rastogi2021self}. Other works are either focused on mitigating the transient faults in SNNs~\cite{putra2021respawn, rastogi2021self} or contemplated permanent fault mitigation in ANN accelerators~\cite{siddique2021exploring, zhang2018analyzing, abdullah2020salvagednn, kundu2020high}. However, when it comes to investigating and mitigating the impact of permanent faults in systolicSNNs, there exists a huge research gap. \textcolor{blue}{This motivates us to investigate the impact of stuck-at 0 and 1 faults on the systolicSNNs and alleviate them through a novel FalVolt mitigation method in this paper.}

\begin{comment}
\begin{figure}[!t]
	\centering
	\vspace{-0.01in}
	\includegraphics[width=0.75\linewidth]{Figs/scnn.pdf}
	\vspace{-0.1in}
	\caption{Spiking Convolutional neural network}
	\label{fig:scnnoverview}
	\vspace{-0.25in}
\end{figure}
\end{comment}

 

%Thus, there is a dire need of extensively investigating and mitigating the impact of faults on systolicSNNs. In this paper, we investigate the impact of stuck-at 0 and 1 faults on the systolicSNNs and mitigate them through a novel FalVolt mitigation method. 



%Hence, there is a huge research gap in analyzing and mitigating the stuck-at faults in systolicSNNs.

%In this paper, we investigate the impact of stuck-at 0 and 1 faults on the systolicSNNs by varying the location of fault bits, number of faulty PEs, and size of systolic arrays. This is the first work that proposes threshold voltage optimization in retraining to mitigate the impact of stuck-at faults on  systolicSNNs. Unlike state-of-the-art works e.g., fault-aware pruning and retraining without threshold voltage optimization which are commonly used for ANNs, FalVolt improves the classification accuracy of systolicSNNs with comparatively less retraining time. 






==> Sections/Sec8_Bibiliography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/Ayesha.jpg}}]{Ayesha Siddique} received her B.Sc. degree in electrical engineering from the Army Public College of Management and Sciences, Rawalpindi, Pakistan, in 2013, and M.S. degree in electrical engineering from the National University of Sciences and Technology (NUST), Islamabad, Pakistan, in 2018. She is currently pursuing her Ph.D. degree in electrical and computer engineering and working as a graduate teaching assistant at the Dependable Cyber-Physical Systems (DCPS) Laboratory in the University of Missouri-Columbia. She also served as a Design Engineer with the Center for Advanced Research in Engineering, Islamabad, Pakistan, from 2013 to 2017. She is a recipient of several awards, including the A. Richard Newton Young Student Fellowship at DAC 2018 and DAC 2020. She is a member of society of women engineers at the University of Missouri-Columbia. Her research interests include reliable and secure neural networks, approximate computing, digital systems design, embedded systems, formal verification and digital image processing.
\end{IEEEbiography}

\vskip -1\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/DrHoque.png}}]{Khaza Anuarul Hoque} received his M.Sc. and Ph.D. degrees from the Department of Electrical and Computer Engineering at Concordia University, Montreal, Canada in 2011 and 2016, respectively. He is currently an Assistant Professor in the Department of Electrical Engineering and Computer Science at the University of Missouri-Columbia (MU) where he directs the Dependable Cyber-Physical Systems (DCPS) Laboratory. His research interests include Cyber-physical and Embedded Systems, Machine Learning, Cybersecurity, and Formal Methods. Before joining MU, he was an FRQNT postdoctoral fellow at the University of Oxford, UK. Dr. Hoque has received several awards and distinctions, including FQRNT Postdoctoral Fellowship Award (2016), FQRNT Doctoral Research Award (2012), and Best Paper Award in 8th IEEE International NEWCAS Conference (2011). He is a senior member of IEEE, and a member of ACM, AAAS, and IEEE Technical Committee on Cyber-Physical Systems (CPS). 
\end{IEEEbiography}

